Semantic Completeness for Correct Maintenance: A Strict Hierarchy of Typing and Inheritance

Removing nominal types or inheritance is defended as reducing burden; cited Java and Go rationales measure no comparison. Correct maintenance minimizes outside answers and repair obligations, preserving required answers and excluding invalid states. Answers identify meanings, memberships, and required implementations. Five capacities form a strict chain. With nominal identities fixed, only multiple contract and implementation parents attain the answer-and-repair optimum on every finite declared history. Incomplete mechanisms force slop: answers restated in code or tooling. In 20 pinned multiple-inheritance Python projects, recovered implementation-class pairs grouped by source class would need outside supply: 12,880 without inheritance, 8,792 under first parents, 739 under sound one-parent optima (checked), zero with multiple parents. With provider and state carriers fixed, state-bearing rows alone force 236 outside pairs. Java and C# interface defaults supply no instance state. At least 24 of 65 size-qualified wheels among the top 150 pure-Python downloads have positive recovered gap (36.9%, 34 unscored). For distinct, independently changing implementations, the ancestry gap is the exact outside-pair minimum with one parent supplying only required pairs, even with reparenting, infinite helpers, delegation, or generators. Zero gap and one-parent contract coverage hold iff class sets nest or are disjoint. Identical records with distinct answers need the confusability graph's chromatic number of keys. Every tree-shaped growth step inserting an off-path provider strictly between ancestors forces one-parent repair. Every snapshot in our constructed history has gap zero, yet repair obligations recur each step; multiple parents add one edge per step. At fixed design costs, bans never lower optima; savings imply suboptimal unrestricted choices.

==> content/notation_macros_auto.tex <==
% Generated from notation.yaml; do not edit.
\RequirePackage{longtable,array,booktabs}
\newif\ifPaperNotationLinks
\PaperNotationLinkstrue
\newif\ifPaperNotationTablePrinted
\DeclareRobustCommand{\PaperNotationLink}[2]{\ensuremath{%
  \ifPaperNotationLinks\hyperlink{paper-notation:#1}{#2}\else#2\fi}}
\AtBeginDocument{%
  \ifdefined\hyperlink\else
    \PackageError{paper-notation}{Linked notation requires hyperref}{Load hyperref in the document preamble.}%
  \fi
  \ifdefined\pdfstringdefDisableCommands
    \pdfstringdefDisableCommands{\def\PaperNotationLink#1#2{#2}}%
  \fi}
\AtEndDocument{%
  \ifPaperNotationTablePrinted\else
    \clearpage
    \section*{Notation (supplementary appendix)}
    \input{content/notation_table_auto.tex}%
  \fi}
\NewDocumentCommand{\PaperClasses}{e{_^}}{\PaperNotationLink{PaperClasses}{C\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperImplementations}{e{_^}}{\PaperNotationLink{PaperImplementations}{F\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperProvider}{e{_^}}{\PaperNotationLink{PaperProvider}{o_f\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperFileReader}{e{_^}}{\PaperNotationLink{PaperFileReader}{\mathrm{FR}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperClassGroup}{e{_^}}{\PaperNotationLink{PaperClassGroup}{A_f\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRequired}{e{_^}}{\PaperNotationLink{PaperRequired}{R^{\mathrm{req}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperPublicRequired}{e{_^}}{\PaperNotationLink{PaperPublicRequired}{R^{\mathrm{req}}_{\mathrm{pub}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperMembership}{e{_^}}{\PaperNotationLink{PaperMembership}{M^{\mathrm{req}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAncestry}{e{_^}}{\PaperNotationLink{PaperAncestry}{H\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRoutes}{e{_^}}{\PaperNotationLink{PaperRoutes}{\varphi\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRoutingStep}{e{_^}}{\PaperNotationLink{PaperRoutingStep}{\to\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRoutingGraph}{e{_^}}{\PaperNotationLink{PaperRoutingGraph}{\Gamma\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRoutingClosure}{e{_^}}{\PaperNotationLink{PaperRoutingClosure}{\to^*\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRemovals}{e{_^}}{\PaperNotationLink{PaperRemovals}{U\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperSupplied}{e{_^}}{\PaperNotationLink{PaperSupplied}{R_D\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperSound}{e{_^}}{\PaperNotationLink{PaperSound}{\mathrm{sound}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperTreeShaped}{e{_^}}{\PaperNotationLink{PaperTreeShaped}{\text{tree-shaped}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperGap}{e{_^}}{\PaperNotationLink{PaperGap}{d_{\downarrow}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperExcess}{e{_^}}{\PaperNotationLink{PaperExcess}{e_H\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRepairSet}{e{_^}}{\PaperNotationLink{PaperRepairSet}{\mathcal D(H,R^{\mathrm{req}})\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRelaxedGap}{e{_^}}{\PaperNotationLink{PaperRelaxedGap}{d_{\lambda}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperOutsideAtState}{e{_^}}{\PaperNotationLink{PaperOutsideAtState}{O_t(D)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperBurden}{e{_^}}{\PaperNotationLink{PaperBurden}{B_{\mathrm{rep}}(n)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperChargedDeletions}{e{_^}}{\PaperNotationLink{PaperChargedDeletions}{\delta\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperOutsideUpdates}{e{_^}}{\PaperNotationLink{PaperOutsideUpdates}{\pi\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperGrowthPairs}{e{_^}}{\PaperNotationLink{PaperGrowthPairs}{\Pi\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperEdgeFootprint}{e{_^}}{\PaperNotationLink{PaperEdgeFootprint}{\operatorname{Through}_t(e)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperMaintenanceIdeal}{e{_^}}{\PaperNotationLink{PaperMaintenanceIdeal}{\operatorname{Maint}^*(\mathcal H)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperSafety}{e{_^}}{\PaperNotationLink{PaperSafety}{\operatorname{Reach}_t(D)\subseteq\operatorname{Valid}_t\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperInput}{e{_^}}{\PaperNotationLink{PaperInput}{X\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAnswerSpace}{e{_^}}{\PaperNotationLink{PaperAnswerSpace}{\mathcal V_{\mathrm{ans}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperEncodingSpace}{e{_^}}{\PaperNotationLink{PaperEncodingSpace}{\mathcal E\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAnswer}{e{_^}}{\PaperNotationLink{PaperAnswer}{a(x)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperConfusability}{e{_^}}{\PaperNotationLink{PaperConfusability}{G^{\mathrm{req}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperKeys}{e{_^}}{\PaperNotationLink{PaperKeys}{\chi(G^{\mathrm{req}})\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperLookup}{e{_^}}{\PaperNotationLink{PaperLookup}{P\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperLookupChoices}{e{_^}}{\PaperNotationLink{PaperLookupChoices}{k\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperSharingQuestions}{e{_^}}{\PaperNotationLink{PaperSharingQuestions}{S\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperDistinctSharing}{e{_^}}{\PaperNotationLink{PaperDistinctSharing}{k_{\sigma,\mathrm{distinct}}\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperInitializationQuestions}{e{_^}}{\PaperNotationLink{PaperInitializationQuestions}{I\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperRecurringCharge}{e{_^}}{\PaperNotationLink{PaperRecurringCharge}{q\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAdoption}{e{_^}}{\PaperNotationLink{PaperAdoption}{K_a\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAdoptionUpkeep}{e{_^}}{\PaperNotationLink{PaperAdoptionUpkeep}{E_a(n)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperAdoptionRate}{e{_^}}{\PaperNotationLink{PaperAdoptionRate}{r_a\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperCommonCost}{e{_^}}{\PaperNotationLink{PaperCommonCost}{K_c(n)\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}
\NewDocumentCommand{\PaperBatchLimit}{e{_^}}{\PaperNotationLink{PaperBatchLimit}{b\IfNoValueF{#1}{_{#1}}\IfNoValueF{#2}{^{#2}}}}


==> external_labels_15b95ee9dc87b1d4.tex <==
% Generated from freshly compiled external-document labels. Do not edit.
% Numbers, pages and titles only: arXiv merges separately compiled PDFs.
\makeatletter
\newlabel{supp-analyzer-new-input}{{9.8.4}{55}{Run the analyzer on another input}{}{}}
\newlabel{supp-anyio-mutation-study}{{9.7}{48}{Displaced-dependency mutation study}{}{}}
\newlabel{supp-anyio-refactoring-application}{{9.6}{46}{An end-to-end AnyIO refactoring decision}{}{}}
\newlabel{supp-atomic-native-completion}{{2}{4}{Required Pairs, Inheritance, and Workarounds}{}{}}
\newlabel{supp-audit-detail}{{9}{42}{Additional Audit Detail}{}{}}
\newlabel{supp-behavioral-substitution}{{4.1}{11}{Behavioral substitution and exact applicability}{}{}}
\newlabel{supp-bounded-realization-cost}{{4.5}{26}{Compression and bounded-capacity realization}{}{}}
\newlabel{supp-charged-deletion-derivation-retention}{{4.1}{23}{Charged deletion is loss of a still-required derivation}{}{}}
\newlabel{supp-charged-work-floor}{{4.2}{16}{Setup-inclusive charged work}{}{}}
\newlabel{supp-checked-kernels}{{13.4}{71}{Checked kernels}{}{}}
\newlabel{supp-claim-handle-mapping}{{16}{110}{Claim-to-Lean Handle Mapping}{}{}}
\newlabel{supp-cooperative-init-order}{{8.2}{40}{Cooperative initialization follows and reverses the MRO}{}{}}
\newlabel{supp-cor:capacity-removal-descent}{{1}{4}{Each missing capacity forces an irreducible semantic obligation}{}{}}
\newlabel{supp-derivation-retention}{{4.5}{23}{Charged deletions interrupt retained derivations}{}{}}
\newlabel{supp-dual-axis-resolution}{{8}{38}{Lookup Order, State Sharing, and Initialization}{}{}}
\newlabel{supp-equal-scope-collapse}{{9.8.2}{51}{Collapsing equal provider scopes}{}{}}
\newlabel{supp-exact-rule-revisions}{{13.3}{70}{Exactly when the rule must change}{}{}}
\newlabel{supp-executable-audits}{{13.5}{73}{Executable audits}{}{}}
\newlabel{supp-explicit-coordinate-parity-menu}{{6}{36}{Explicit Coordinate-and-Parity Menu}{}{}}
\newlabel{supp-external-route-control}{{9.8.5}{56}{External-route syntax control}{}{}}
\newlabel{supp-fig:abstract-concrete-boundary}{{3}{56}{A five-class abstract/concrete boundary witness. Coverage is forced when one incomparable candidate supplies the queried member; genuinely competing concrete declarations remain unattributed}{}{}}
\newlabel{supp-fig:skewed-crossing-probability}{{2}{34}{At the audited component size $n=256$, the green source reaches only 5\% because one crossing cell is suppressed by 99.92\% (1,248$\times $ below balanced). With positive support in all three crossing cells, a crossing eventually appears with probability approaching one; skew changes its arrival time}{}{}}
\newlabel{supp-fig:storage-encodings}{{1}{30}{Same shown outputs, different facts for code to maintain as providers evolve. Inheritance derives both pairs; fields need routes. The monolith loses \texttt {MixA} and \texttt {MixB}'s required independent identities}{}{}}
\newlabel{supp-finite-identity-policies}{{3}{9}{Proofs for the Finite Identity Policies}{}{}}
\newlabel{supp-finite-rule-generation}{{13.2}{68}{When finite lookup code can generate the complete provider list}{}{}}
\newlabel{supp-fixed-top-routing}{{4.3}{22}{Parked-top policy: standing supply without fresh repairs}{}{}}
\newlabel{supp-formalization-boundary}{{13}{67}{What the Proofs and Executable Checks Establish}{}{}}
\newlabel{supp-go-direct-method-history}{{12}{66}{Go Direct-Method History and Deletion Counterfactual}{}{}}
\newlabel{supp-history-rewrite-screen}{{9.5}{45}{History screen for MI-to-SI rewrites}{}{}}
\newlabel{supp-immediate-parent-evolution}{{4.3}{18}{Immediate-parent evolution}{}{}}
\newlabel{supp-independent-outside-bundles}{{4.2}{15}{Independent outside bundles}{}{}}
\newlabel{supp-java-forwarding-check}{{9.8.6}{57}{Java forwarding check}{}{}}
\newlabel{supp-known-schema-families}{{7}{37}{Known Schema Families and Lattice Closure}{}{}}
\newlabel{supp-language-encodings}{{14}{74}{Representative Language Encodings of the Factorization Gap}{}{}}
\newlabel{supp-lean-handle-ledger}{{15}{79}{Full Lean Handle Ledger}{}{}}
\newlabel{supp-linear-field-menu-bounds}{{5}{36}{Linear Field-Menu Bounds}{}{}}
\newlabel{supp-longitudinal-completion}{{9.2}{44}{Workaround changes under the declared first-parent policy}{}{}}
\newlabel{supp-minimum-one-parent-completion}{{2.2}{8}{Minimum one-parent workaround count}{}{}}
\newlabel{supp-monotone-multiparent-attainment}{{4.5}{24}{Joint attainment on arbitrary finite supply histories}{}{}}
\newlabel{supp-notation}{{}{1}{Notation}{}{}}
\newlabel{supp-omission-tolerance-gap}{{9.2}{59}{Omission tolerance saves at most one answer per tolerated pair}{}{}}
\newlabel{supp-paper-claim-location:1}{{1}{4}{Each missing capacity forces an irreducible semantic obligation}{}{}}
\newlabel{supp-paper-claim-location:10}{{10}{13}{Valid overrides keep promised calls available}{}{}}
\newlabel{supp-paper-claim-location:100}{{94}{59}{Declared tolerance: a third cell value}{}{}}
\newlabel{supp-paper-claim-location:101}{{9.9}{59}{Declared tolerance: a third cell value}{}{}}
\newlabel{supp-paper-claim-location:102}{{95}{59}{Omission tolerance saves at most one answer per tolerated pair}{}{}}
\newlabel{supp-paper-claim-location:103}{{96}{60}{Declared tolerance: a third cell value}{}{}}
\newlabel{supp-paper-claim-location:104}{{97}{61}{Weighted and fixed-forest factorization objectives}{}{}}
\newlabel{supp-paper-claim-location:105}{{98}{64}{TypeScript Published-Brand History Audit}{}{}}
\newlabel{supp-paper-claim-location:106}{{99}{67}{Answer counts do not depend on a source-length convention}{}{}}
\newlabel{supp-paper-claim-location:107}{{100}{67}{What single-omission checks must exercise}{}{}}
\newlabel{supp-paper-claim-location:108}{{101}{67}{What single-omission checks must exercise}{}{}}
\newlabel{supp-paper-claim-location:109}{{102}{67}{What single-omission checks must exercise}{}{}}
\newlabel{supp-paper-claim-location:11}{{11}{13}{Declared property instances}{}{}}
\newlabel{supp-paper-claim-location:110}{{13.1}{68}{Rules can supply future pairs without new manual wiring}{}{}}
\newlabel{supp-paper-claim-location:111}{{103}{68}{One rule can generate exact ancestry at every input}{}{}}
\newlabel{supp-paper-claim-location:112}{{13.2}{68}{When finite lookup code can generate the complete provider list}{}{}}
\newlabel{supp-paper-claim-location:113}{{104}{68}{Exact condition for complete provider-list generation}{}{}}
\newlabel{supp-paper-claim-location:114}{{13.2}{69}{When finite lookup code can generate the complete provider list}{}{}}
\newlabel{supp-paper-claim-location:115}{{105}{69}{One possible answer per class still need not be listable}{}{}}
\newlabel{supp-paper-claim-location:116}{{106}{70}{Python correspondence}{}{}}
\newlabel{supp-paper-claim-location:117}{{13.3}{70}{Exactly when the rule must change}{}{}}
\newlabel{supp-paper-claim-location:118}{{107}{70}{Exact rule-revision count on a finite history}{}{}}
\newlabel{supp-paper-claim-location:119}{{108}{71}{Exactly when the rule must change}{}{}}
\newlabel{supp-paper-claim-location:12}{{12}{13}{Declared property instances}{}{}}
\newlabel{supp-paper-claim-location:120}{{109}{71}{Exactly when the rule must change}{}{}}
\newlabel{supp-paper-claim-location:121}{{110}{72}{Checked kernels}{}{}}
\newlabel{supp-paper-claim-location:122}{{111}{72}{Checked kernels}{}{}}
\newlabel{supp-paper-claim-location:123}{{112}{72}{Checked kernels}{}{}}
\newlabel{supp-paper-claim-location:124}{{113}{73}{Checked kernels}{}{}}
\newlabel{supp-paper-claim-location:125}{{114}{73}{Checked kernels}{}{}}
\newlabel{supp-paper-claim-location:126}{{115}{74}{Representative Language Encodings of the Factorization Gap}{}{}}
\newlabel{supp-paper-claim-location:13}{{13}{13}{Uncomputability of unrestricted structural safety}{}{}}
\newlabel{supp-paper-claim-location:14}{{14}{14}{Uncomputability of unrestricted structural safety}{}{}}
\newlabel{supp-paper-claim-location:15}{{15}{14}{Uncomputability of unrestricted structural safety}{}{}}
\newlabel{supp-paper-claim-location:16}{{16}{14}{Uncomputability of unrestricted structural safety}{}{}}
\newlabel{supp-paper-claim-location:17}{{17}{14}{Open-world one-parent adequacy}{}{}}
\newlabel{supp-paper-claim-location:18}{{18}{14}{Open-world one-parent adequacy}{}{}}
\newlabel{supp-paper-claim-location:19}{{19}{15}{Finite tests and their trust boundary}{}{}}
\newlabel{supp-paper-claim-location:2}{{2}{7}{Required Pairs, Inheritance, and Workarounds}{}{}}
\newlabel{supp-paper-claim-location:20}{{20}{15}{Matching-coarsening recourse}{}{}}
\newlabel{supp-paper-claim-location:21}{{21}{15}{Explicit field-menu translation}{}{}}
\newlabel{supp-paper-claim-location:22}{{22}{15}{Two and three known states}{}{}}
\newlabel{supp-paper-claim-location:23}{{23}{15}{Minimum replacement state}{}{}}
\newlabel{supp-paper-claim-location:24}{{24}{15}{Independent outside bundles}{}{}}
\newlabel{supp-paper-claim-location:25}{{25}{16}{Independent outside bundles}{}{}}
\newlabel{supp-paper-claim-location:26}{{26}{16}{Setup-inclusive charged work}{}{}}
\newlabel{supp-paper-claim-location:27}{{27}{16}{Setup-inclusive charged work}{}{}}
\newlabel{supp-paper-claim-location:28}{{28}{16}{Setup-inclusive charged work}{}{}}
\newlabel{supp-paper-claim-location:29}{{29}{17}{Adding unrelated pairs leaves the gap fixed while shrinking its fraction}{}{}}
\newlabel{supp-paper-claim-location:3}{{3}{8}{Exact semantic factoring}{}{}}
\newlabel{supp-paper-claim-location:30}{{30}{17}{Proof detail for keys after name erasure}{}{}}
\newlabel{supp-paper-claim-location:31}{{31}{17}{Minimum reusable adapters}{}{}}
\newlabel{supp-paper-claim-location:32}{{32}{17}{Choosing one authoritative declaration per role}{}{}}
\newlabel{supp-paper-claim-location:33}{{33}{17}{Choosing one authoritative declaration per role}{}{}}
\newlabel{supp-paper-claim-location:34}{{34}{17}{Choosing one authoritative declaration per role}{}{}}
\newlabel{supp-paper-claim-location:35}{{35}{18}{Role-normalization direction}{}{}}
\newlabel{supp-paper-claim-location:36}{{36}{18}{Exact supply forbids over-coverage}{}{}}
\newlabel{supp-paper-claim-location:37}{{37}{18}{Exact supply forbids over-coverage}{}{}}
\newlabel{supp-paper-claim-location:38}{{38}{19}{Immediate-parent evolution}{}{}}
\newlabel{supp-paper-claim-location:39}{{39}{19}{Immediate-parent evolution}{}{}}
\newlabel{supp-paper-claim-location:4}{{4}{8}{Minimum one-parent workaround count}{}{}}
\newlabel{supp-paper-claim-location:40}{{40}{19}{Immediate-parent evolution}{}{}}
\newlabel{supp-paper-claim-location:41}{{41}{20}{Immediate-parent evolution}{}{}}
\newlabel{supp-paper-claim-location:42}{{42}{20}{Immediate-parent evolution}{}{}}
\newlabel{supp-paper-claim-location:43}{{43}{20}{Missing and unwanted pairs split into forced gap and removable excess}{}{}}
\newlabel{supp-paper-claim-location:44}{{44}{21}{Successful outputs and ancestry cannot reveal the gap}{}{}}
\newlabel{supp-paper-claim-location:45}{{45}{21}{Successful outputs and ancestry cannot reveal the gap}{}{}}
\newlabel{supp-paper-claim-location:46}{{46}{21}{Capacity-removal descent}{}{}}
\newlabel{supp-paper-claim-location:47}{{47}{21}{Ignoring workaround costs reverses the choice}{}{}}
\newlabel{supp-paper-claim-location:48}{{48}{22}{Parked-top policy: standing supply without fresh repairs}{}{}}
\newlabel{supp-paper-claim-location:49}{{49}{22}{Admission checks for fresh routing configurations}{}{}}
\newlabel{supp-paper-claim-location:5}{{5}{9}{Adding identity evidence after a collision}{}{}}
\newlabel{supp-paper-claim-location:50}{{50}{23}{Admission checks for fresh routing configurations}{}{}}
\newlabel{supp-paper-claim-location:51}{{4.5}{23}{Charged deletions interrupt retained derivations}{}{}}
\newlabel{supp-paper-claim-location:52}{{51}{23}{Charged deletion is loss of a still-required derivation}{}{}}
\newlabel{supp-paper-claim-location:53}{{52}{24}{Charged deletions interrupt retained derivations}{}{}}
\newlabel{supp-paper-claim-location:54}{{53}{24}{Joint attainment on arbitrary finite supply histories}{}{}}
\newlabel{supp-paper-claim-location:55}{{54}{24}{Joint attainment on arbitrary finite supply histories}{}{}}
\newlabel{supp-paper-claim-location:56}{{4.5}{24}{Exactly which accountings preserve the strict separations}{}{}}
\newlabel{supp-paper-claim-location:57}{{55}{24}{Every crossing survives exactly when nonempty outside work costs positively}{}{}}
\newlabel{supp-paper-claim-location:58}{{4.5}{25}{Exactly which accountings preserve the strict separations}{}{}}
\newlabel{supp-paper-claim-location:59}{{56}{25}{Strict separations survive non-additive prices}{}{}}
\newlabel{supp-paper-claim-location:6}{{6}{9}{Retaining names cannot increase extra-key demand}{}{}}
\newlabel{supp-paper-claim-location:60}{{4.5}{25}{Every faithful representation must realize a semantic change}{}{}}
\newlabel{supp-paper-claim-location:61}{{57}{26}{A semantic change requires positively priced execution}{}{}}
\newlabel{supp-paper-claim-location:62}{{58}{26}{Compression and bounded-capacity realization}{}{}}
\newlabel{supp-paper-claim-location:63}{{59}{27}{Compression and bounded-capacity realization}{}{}}
\newlabel{supp-paper-claim-location:64}{{60}{27}{Learning belongs in the policy comparison}{}{}}
\newlabel{supp-paper-claim-location:65}{{61}{28}{Optimum versus realized choice}{}{}}
\newlabel{supp-paper-claim-location:66}{{62}{28}{Optimum versus realized choice}{}{}}
\newlabel{supp-paper-claim-location:67}{{63}{28}{Tools must supply every missing implementation--class pair}{}{}}
\newlabel{supp-paper-claim-location:68}{{64}{29}{Assignment expressions separate local rewrites from whole-program repairs}{}{}}
\newlabel{supp-paper-claim-location:69}{{65}{29}{Assignment expressions separate local rewrites from whole-program repairs}{}{}}
\newlabel{supp-paper-claim-location:7}{{7}{9}{Retaining names cannot increase extra-key demand}{}{}}
\newlabel{supp-paper-claim-location:70}{{66}{29}{Assignment expressions separate local rewrites from whole-program repairs}{}{}}
\newlabel{supp-paper-claim-location:71}{{67}{30}{Assignment expressions separate local rewrites from whole-program repairs}{}{}}
\newlabel{supp-paper-claim-location:72}{{68}{31}{Invalid-state necessity}{}{}}
\newlabel{supp-paper-claim-location:73}{{69}{31}{Invalid-state necessity}{}{}}
\newlabel{supp-paper-claim-location:74}{{70}{31}{Time-weighted acquisition costs}{}{}}
\newlabel{supp-paper-claim-location:75}{{71}{32}{Exact two-role and row--column gaps}{}{}}
\newlabel{supp-paper-claim-location:76}{{72}{32}{Exact two-role and row--column gaps}{}{}}
\newlabel{supp-paper-claim-location:77}{{73}{33}{Arbitrary skew and changing population size}{}{}}
\newlabel{supp-paper-claim-location:78}{{74}{35}{Arbitrary skew and changing population size}{}{}}
\newlabel{supp-paper-claim-location:79}{{75}{35}{Fixed-description factoring statement}{}{}}
\newlabel{supp-paper-claim-location:8}{{8}{11}{One answer-preservation condition across the models}{}{}}
\newlabel{supp-paper-claim-location:80}{{76}{36}{Exact expansion preserves the valid domain}{}{}}
\newlabel{supp-paper-claim-location:81}{{77}{36}{Linear Field-Menu Bounds}{}{}}
\newlabel{supp-paper-claim-location:82}{{78}{39}{Supply and winner selection count different answers}{}{}}
\newlabel{supp-paper-claim-location:83}{{79}{39}{One graph can couple otherwise separate relations}{}{}}
\newlabel{supp-paper-claim-location:84}{{80}{39}{Self-use reverses the native winner default}{}{}}
\newlabel{supp-paper-claim-location:85}{{81}{39}{Coherent resolution is one precedence order}{}{}}
\newlabel{supp-paper-claim-location:86}{{82}{40}{Coherent resolution is one precedence order}{}{}}
\newlabel{supp-paper-claim-location:87}{{83}{40}{Coherent resolution is one precedence order}{}{}}
\newlabel{supp-paper-claim-location:88}{{84}{40}{Specified state answers survive answer-preserving refactoring}{}{}}
\newlabel{supp-paper-claim-location:89}{{8.1}{40}{State sharing and cooperative initialization}{}{}}
\newlabel{supp-paper-claim-location:9}{{9}{12}{Behavioral substitution and exact applicability}{}{}}
\newlabel{supp-paper-claim-location:90}{{85}{40}{Cooperative initialization follows and reverses the MRO}{}{}}
\newlabel{supp-paper-claim-location:91}{{86}{41}{A shared-state default prices distinct-state exceptions}{}{}}
\newlabel{supp-paper-claim-location:92}{{87}{41}{Lookup and initialization can require one outside answer}{}{}}
\newlabel{supp-paper-claim-location:93}{{88}{42}{State requirements preserve capacity containment}{}{}}
\newlabel{supp-paper-claim-location:94}{{89}{43}{SQLAlchemy's largest independently certified component}{}{}}
\newlabel{supp-paper-claim-location:95}{{90}{45}{Preregistered strict-insertion history audit}{}{}}
\newlabel{supp-paper-claim-location:96}{{91}{49}{Omitted requirements can raise or lower the gap}{}{}}
\newlabel{supp-paper-claim-location:97}{{92}{51}{Public-name preservation contract}{}{}}
\newlabel{supp-paper-claim-location:98}{{9.8.2}{54}{Provider state in archived optimal repairs}{}{}}
\newlabel{supp-paper-claim-location:99}{{93}{54}{Restricting provider rows bounds the stateful gap}{}{}}
\newlabel{supp-price-invariant-separations}{{4.5}{24}{Exactly which accountings preserve the strict separations}{}{}}
\newlabel{supp-prop:exact-rule-revisions}{{13.4}{70}{Exact rule-revision count on a finite history}{}{}}
\newlabel{supp-prop:finite-rule-generation}{{13.2}{68}{Exact condition for complete provider-list generation}{}{}}
\newlabel{supp-prop:rule-generated-ancestry}{{13.1}{68}{One rule can generate exact ancestry at every input}{}{}}
\newlabel{supp-prop:singleton-provider-separation}{{13.3}{69}{One possible answer per class still need not be listable}{}{}}
\newlabel{supp-protobuf-audit}{{10}{62}{Protocol Buffer Permanent-Key Audit}{}{}}
\newlabel{supp-provider-state-audit}{{9.8.2}{51}{Provider state in archived optimal repairs}{}{}}
\newlabel{supp-pyappkit-portfolio}{{9.4}{45}{Pinned pyapp-kit portfolio}{}{}}
\newlabel{supp-python-extraction-strengthening}{{9.8.3}{54}{Recovering unique concrete bodies among abstract declarations}{}{}}
\newlabel{supp-python-factorization-results}{{9.9}{58}{Python factorization results and certificates}{}{}}
\newlabel{supp-python-population-protocol}{{9.8}{49}{Python population selection and extraction protocol}{}{}}
\newlabel{supp-python-public-api-contract}{{9.8.1}{50}{Public-name preservation contract}{}{}}
\newlabel{supp-relaxed-supply-proof}{{4}{11}{Relaxed-supply proof}{}{}}
\newlabel{supp-repair-retention-pricing}{{4.5}{23}{Pricing repair and retention}{}{}}
\newlabel{supp-scope-ledger}{{1}{4}{What Each Result Counts}{}{}}
\newlabel{supp-sec:completion-admission-audit}{{4.4}{22}{Admission checks for fresh routing configurations}{}{}}
\newlabel{supp-sec:rule-based-factoring}{{13.1}{67}{Rules can supply future pairs without new manual wiring}{}{}}
\newlabel{supp-semantic-change-positive-cost}{{4.5}{25}{Every faithful representation must realize a semantic change}{}{}}
\newlabel{supp-semantic-deletion-normalization}{{4.5}{23}{Semantic deletions do not create repair obligations}{}{}}
\newlabel{supp-semantic-factoring}{{2.1}{7}{Exact semantic factoring}{}{}}
\newlabel{supp-sharing-default-exceptions}{{8.3}{41}{A shared-state default prices distinct-state exceptions}{}{}}
\newlabel{supp-sqlalchemy-component}{{9.1}{43}{SQLAlchemy's largest independently certified component}{}{}}
\newlabel{supp-state-answer-invariance}{{8.1}{40}{Specified state answers survive answer-preserving refactoring}{}{}}
\newlabel{supp-state-capacity-containment}{{8.5}{42}{State requirements preserve capacity containment}{}{}}
\newlabel{supp-state-coordination}{{8.1}{40}{State sharing and cooperative initialization}{}{}}
\newlabel{supp-state-lookup-coupling}{{8.4}{41}{Lookup and initialization can require one outside answer}{}{}}
\newlabel{supp-stateful-row-projection-bound}{{9.1}{54}{Restricting provider rows bounds the stateful gap}{}{}}
\newlabel{supp-strict-insertion-audit}{{9.3}{44}{Preregistered strict-insertion history audit}{}{}}
\newlabel{supp-supp:acquisition-policy-optimality}{{4.6}{27}{Learning belongs in the policy comparison}{}{}}
\newlabel{supp-supp:tooling-completion}{{4.7}{28}{Tools must supply every missing implementation--class pair}{}{}}
\newlabel{supp-supp:walrus-boundary}{{4.7}{28}{Assignment expressions separate local rewrites from whole-program repairs}{}{}}
\newlabel{supp-tab:anyio-mutation}{{12}{49}{AnyIO mutation outcomes for all \MutationDenominator {} generated single omissions. The baseline passed \MutationBaselinePassed {} tests, and the pinned suite detected all \MutationDetected {} omissions}{}{}}
\newlabel{supp-tab:audit-scope-ledger}{{8}{42}{Fixed inputs, evidence, and boundaries of the inheritance audits}{}{}}
\newlabel{supp-tab:claim-lean-handle-mapping}{{30}{111}{Claim-to-Lean handle mapping}{}{}}
\newlabel{supp-tab:cost-units}{{4}{7}{The paper keeps distinct quantities in distinct units. Source lines, human time, and comprehension enter only when a stated model measures them}{}{}}
\newlabel{supp-tab:derivation-scope-supp}{{3}{6}{Scope of the derivation results. Paid removal relaxes exact supply without changing the required-only inheritance theorem or permitting promise-blocking}{}{}}
\newlabel{supp-tab:equal-scope-collapse}{{15}{53}{Equal-scope relaxation on the locked twenty-project cohort. Only identical class sets merge; every quotient optimum is independently certified}{}{}}
\newlabel{supp-tab:external-route-controls}{{18}{57}{Route-spelling crossings among \ExternalRouteControlPositive {} of \ExternalRouteControlEligible {} size-qualified zero-local-MI wheels. Each row's two member spellings share the field name recorded in the verified JSON. The final column applies the two-role formula $\min \{N_{10},N_{11},N_{01}\}=1$ to this syntactic relation. Provider resolution rejects every candidate: matching spellings either use distinct providers or omit inherited routes, which resolves the apparent crossings}{}{}}
\newlabel{supp-tab:history-rewrite-screen}{{11}{46}{Locked mainline syntax screen for the five largest positive provider-bundle gaps. The scan finds 13 relocated nominal factors in total; the table reports candidate, commit, parser-failure, and fallback counts by project. Historical files outside the parser model remain counted as parse failures}{}{}}
\newlabel{supp-tab:lean-handle-index}{{29}{80}{Lean handle index}{}{}}
\newlabel{supp-tab:property-instances-supp}{{5}{13}{Instances of the shared boundary contract. The safety, availability, and liveness rows characterize preservation of the declared answer; they do not add latency, probability, scheduler, or fairness claims not present in the row's inputs. All rows instantiate the generic Lean theorem BPI1; the projection row additionally uses PJD1--4 for its exact-recovery/non-extraction duality}{}{}}
\newlabel{supp-tab:public-api-contract}{{14}{52}{Separate public-name resolution contract on the original twenty projects. Dunders count as public; provider declarations may be private. Zero-pair rows are retained}{}{}}
\newlabel{supp-tab:pyappkit-portfolio}{{10}{46}{All libraries on the pinned pyapp-kit landing page. ``External MI'' counts multi-parent classes with at least one unresolved direct base. The exact gap prices the source-local provider map and therefore excludes those external branches}{}{}}
\newlabel{supp-tab:python-cpsat-trust}{{19}{59}{Archived OR-Tools CP-SAT 9.15.6755 search results for the seven components with independent Lean-checked LRAT lower bounds. Primary component indices are zero-based; ``\PaperNotationLink {PaperClasses}{C}3 max'' is the maximum-gap fully local Closed-\PaperNotationLink {PaperClasses}{C}3 subcomponent. The independent checker reparses each retained-laminar witness. The archived solver status is not a premise of exactness}{}{}}
\newlabel{supp-tab:python-extraction-strengthening}{{17}{56}{Frozen-rule versus strengthened-rule extraction. ``Ambiguities'' is before--after. Equal relation digests are recorded in the complete JSON; the displayed digest is the strengthened relation's SHA-256 prefix}{}{}}
\newlabel{supp-tab:python-method-sensitivity}{{22}{60}{Method-slot sensitivity by project. The method gap is the pinned solver optimum when the reported status is \texttt {OPTIMAL}; otherwise the entry is the checked lower--upper interval. Solver optimality remains inside the declared trust boundary}{}{}}
\newlabel{supp-tab:python-specification-sensitivity}{{20}{60}{Specification and removal sensitivities. Each interval gives a solver lower bound and a checked supply-repair upper bound. For unit removal cost, the aggregate upper repair contains \PythonPaidBlockingForwarded {} forwarded pairs and \PythonPaidBlockingBlocked {} removed pairs}{}{}}
\newlabel{supp-tab:result-scope-supp}{{2}{5}{Scope of the identity-capacity results. Only the last four rows use coordinate-set profiles; the earlier rows range over abstract observation equivalences}{}{}}
\newlabel{supp-tab:rule-based-python}{{26}{70}{One family rule, four Python routes. All four preserve separate class identities and use the same descriptor providers. Class creation and its required input still occur; an unchanged rule removes repeated wiring edits}{}{}}
\newlabel{supp-tab:skewed-crossing-thresholds}{{6}{34}{Exact waiting thresholds under skew. The four cells are neither, left only, right only, and both. $n_{\alpha }$ is the first population size with $\Pr [d_\downarrow >0]\ge \alpha $}{}{}}
\newlabel{supp-tab:skewed-gap-severity}{{7}{35}{Exact gap severity under the same skewed sources. Skew changes the waiting time and slope while each displaced pair remains one outside semantic answer}{}{}}
\newlabel{supp-tab:stateful-provider-gap}{{16}{55}{State-bearing provider rows, with fixed identities, scopes, and sound ancestry. The upper column restricts the primary repair; the exact column reoptimizes this subrelation. Components of gap at most 10 use exhaustive replay; larger ones use Lean-checked LRAT}{}{}}
\newlabel{supp-tab:supp-documented-completion-artifacts}{{28}{78}{Primary-source instances of the carrier, replacement, overreach, relation-splitting, and external-authority cases. The classification is a consequence of the fixed-relation model: shipped behavior determines the case, and the platform's reasons for choosing it are a separate historical question}{}{}}
\newlabel{supp-tab:supp-language-carriers}{{27}{75}{Representative native carriers for implementation applicability. These carriers locate the coordinatewise correct-maintenance capacities in the main-text mechanism table; precedence and separate answers remain part of each placement}{}{}}
\newlabel{supp-tab:supp-protobuf-key-seven}{{23}{63}{An end-to-end reuse certificate from the pinned Protocol Buffer history. The schema-slot key is (message, field number)}{}{}}
\newlabel{supp-tab:typescript-brand-history}{{24}{65}{Pinned TypeScript brand-history receipt. Prices are exact for the sampled package-local graphs. A latest price of zero means that the latest sampled release exposes no meaning in the extracted relation; it does not erase earlier conflicts from the history contract}{}{}}
\newlabel{supp-thm:accounting-characterization}{{4.2}{24}{Every crossing survives exactly when nonempty outside work costs positively}{}{}}
\newlabel{supp-thm:price-invariant-separations}{{4.3}{25}{Strict separations survive non-additive prices}{}{}}
\newlabel{supp-thm:semantic-change-positive-cost}{{4.4}{26}{A semantic change requires positively priced execution}{}{}}
\newlabel{supp-time-weighted-acquisition}{{4.8}{31}{Time-weighted acquisition costs}{}{}}
\newlabel{supp-two-role-row-column-gaps}{{4.9}{32}{Exact two-role and row--column gaps}{}{}}
\newlabel{supp-typescript-brand-audit}{{11}{63}{TypeScript Published-Brand History Audit}{}{}}
\makeatother

